Individual Fairness for $k$-Clustering

We give a local search based algorithm for $k$-median and $k$-means (and more generally for any $k$-clustering with $\ell_p$ norm cost function) from the perspective of individual fairness. More precisely, for a point $x$ in a point set $P$ of size $n$, let $r(x)$ be the minimum radius such that the ball of radius $r(x)$ centered at $x$ has at least $n/k$ points from $P$. Intuitively, if a set of $k$ random points are chosen from $P$ as centers, every point $x\in P$ expects to have a center within radius $r(x)$. An individually fair clustering provides such a guarantee for every point $x\in P$. This notion of fairness was introduced in [Jung et al., 2019] where they showed how to get an approximately feasible $k$-clustering with respect to this fairness condition. In this work, we show how to get a bicriteria approximation for fair $k$-clustering: The $k$-median ($k$-means) cost of our solution is within a constant factor of the cost of an optimal fair $k$-clustering, and our solution approximately satisfies the fairness condition (also within a constant factor). Further, we complement our theoretical bounds with empirical evaluation.

==> k-means.tex <==
\section{Fair Algorithms for $k$-Means}
\subsection{Analysis of Local Search for Fair $k$-Means}\label{sec:k-means}
The local search algorithm for $\alpha$-fair $k$-means is similar to the one with $k$-median objective function and was first analyzed by~\cite{kanungo2004local} for Euclidean space using a so-called ``centroidal'' property of optimal solutions in $k$-means. Later, the analysis both simplified and generalized by~\cite{gupta2008simpler}; their analysis showed that local search algorithm works for $k$-means in general metric spaces.

In this section, as in the analysis of $k$-median (Section~\ref{sec:k-median}), we assume the existence of a $\Delta$-bounded mapping $\pi$ and $(t,\gamma)$-bounded covering of the edges of $\pi$, $\sQ$ (see Section~\ref{sec:mapping-covering} for more details on the bounded mapping and covering). With this assumption, we can show that if the local search algorithm stops at time $T$, the $k$-means cost clustering of the point set $P$ using the centers at time $T$, $S$ is within a constant factor of the cost of an optimal $\alpha$-fair $k$-means of the point set $P$. Note that by the termination condition of the local search algorithm, $S$ is a $(t,\eps)$-stable set of centers.
 
In the rest of this section, we use $\d(x,y)$ to denote the squared distance of $x$ and $y$; $\d(x,y) := d(x,y)^2$.  
%\avnote{High-level approach is similar to the one by David Mount et al.}
\begin{lemma}\label{lem:means-constant}
Consider a set of $n$ points $P$ in a metric space $(X, d)$. Let $O$ be a set of centers for an optimal $\alpha$-fair $k$-means of $P$ and let $S$ be a set of $(t, \eps)$-stable $k$ centers for which there exists a pair of $\Delta$-bounded mapping $\pi: O\rightarrow S$ and $(t, \gamma)$-bounded covering $\sQ$. Then, $\cost(S) \leq  4\gamma^2\cdot (4\Delta+1)^2 \cdot \opt$ where $\opt$ denotes the cost of an optimal $\alpha$-fair $k$-means of $P$ (i.e., the $k$-means cost using $O$ as centers).  
\end{lemma}
\begin{proof}
Consider an arbitrary partition $Q \in \sQ$. %Similarly to the approach of~\cite{arya2004local} and \cite{kanungo2004local}, 
Here, we bound the difference between the $k$-means cost of $P$ with the set $S$ as centers and the set $S_Q = (S\cup O(Q))\setminus{S(Q)}$ as centers. 

Let $S_j\subseteq P$ denote the cluster of points that are mapped to $s_j$ in the clustering with the set $S$ as centers and let $O_i\subseteq P$ denote the cluster of points that are mapped to $o_i$ in the clustering with the set $O$ as centers. Moreover, we use $\sO_Q$ and $\sS_Q$ respectively to denote $\bigcup_{o_i\in O(Q)} O_i$ and $\bigcup_{s_j\in S(Q)} S_j$.
\begin{align}
\sum_{x\in P} \d(x, S_Q) - \d(x, S) 
	&\leq \sum_{x\in \sO_Q} \d(x, S_Q) -  \d(x, S) + \sum_{x\in \sS_Q \setminus \sO_Q} \d(x, S_Q) - \d(x, S)  \nonumber \\
	&\leq \sum_{x\in \sO_Q} \d(x, o_x) - \d(x, s_x) &&\rhd o_x=\nn_O(x), s_x = \nn_S(x) \nonumber \\ 
	&+ \sum_{x\in \sS_Q \setminus \sO_Q} \d(x, s_{o_x}) - \d(x, s_x) &&\rhd s_{o_x}= \nn_S(o_x) \label{eq:means_cost_of_swap}
\end{align}
By summing over all partitions $Q\in \sQ$, 
\begin{align}
\sum_{Q\in \sQ} \sum_{x\in P} \d(x, S_Q) - \d(x, S) 
	&\leq \sum_{Q\in \sQ} \Big( \sum_{x\in \sO_Q} \big( \d(x, o_x) - \d(x, s_x)\big) + \sum_{x\in \sS_Q \setminus \sO_Q} \big( \d(x, s_{o_x}) - \d(x, s_x) \big) \Big) \nonumber\\ 
	&\leq \gamma\cdot \opt - \cost(S) \nonumber + \gamma\cdot \Delta \cdot (\sum_{x\in P} \d(x, s_{o_x}) - \d(x, s_x)) \\
	&\leq \gamma\cdot \opt - (\gamma\cdot\Delta + 1) \cdot \cost(S) + \gamma\cdot \Delta \cdot \sum_{x\in P} \d(x, s_{o_x}) \label{eq:final-bound} 
\end{align}
where the second inequality follows from Property~D-\ref{enum:mapping-2} and Property~E-\ref{enum:partition-0} of $(\pi, \sQ)$ and the third inequality follows from the fact that given $S_j$, for all $x\in S_j$, $\d(x, s_{o_x}) - \d(x, s_j) \geq 0$. 

Next, we will bound the term $\sum_{x\in P} \d(x, s_{o_x})$ in Eq.~\eqref{eq:final-bound}.
\begin{claim}\label{clm:bound-R-term}
Let $s_{o_x}$ be the nearest center in $S$ to $o_x$ where $o_x$ is the nearest center in $O$ to $x$. Assuming $\beta^2 = {\cost(S) / \opt}$, then $\sum_{x\in P} \d(x, s_{o_x}) \leq (2+\beta)^2\cdot \opt$.
\end{claim} 
\begin{proof}
Let $p_1, \cdots, p_n$ denote the points in $P$. We define vector $\X$ so that the $i$-th coordinate in $\X_i$ is equal to $d(p_i, o_{p_i})$. Similarly, we define $\Y$ so that $\Y_i = d(p_i, s_{p_i})$. Note that in particular, $\left\| 2\X \right\|_2^2 = 4\cdot \opt$ and $\left\| \Y \right\|_2^2 = \cost(S)$.
\begin{align*}
\sum_{x\in P} \d(x, s_{o_x}) 
&\leq \sum_{x\in P} (2d(x, o_x) + d(x, s_x))^2 \;\rhd\text{by Eq.~\eqref{eq:closest-stable-center}}\\
&= \left\|2\X + \Y \right\|_2^2\\
&\leq \big(\left\| 2\X \right\|_2 + \left\| \Y \right\|_2\big)^2 \; \rhd\text{triangle inequality (Minkowski inequality on $L^p$ with $p>1$)}\\
&\leq (2\sqrt{\opt} + \sqrt{\cost(S)})^2 \\
&\leq (2+\beta)^2\cdot \opt \;\rhd\text{by $\beta^2 = {\cost(S) / \opt}$}
%&= \sum_{o_i\in O} \sum_{x\in O_i} \d(x,s_{o_i}) \\
%&= \sum_{o_i \in O} \d(O_i, s_{o_i}) \\
%&\leq \sum_{o_i \in O} \d(O_i, o_i) + |O_i|\cdot \d(o_i, s_{o_i}) &&\rhd\text{centroid property of $k$-means clustering} \\
%&= \sum_{o_i\in O} \sum_{x\in O_i} \d(x, o_i) + \d(o_i, s_{o_i}) \\ 
%&\leq \sum_{o_i\in O} \sum_{x\in O_i} \d(x, o_i) + \d(o_i, s_{x}) \\
%&= \sum_{x\in P} \d(x, o_{x}) + \d(o_{x}, s_{x}) \\
%&\leq \sum_{x\in P} \d(x, o_{x}) + (d(x, o_{x}) + d(x, s_{x}))^2 &&\rhd\text{triangle inequality} \\
%&= \sum_{x\in P} 2\cdot \d(x, o_{x}) + \d(x, s_x) + 2\cdot d(x, o_{x}) \cdot d(x, s_{x}) \\
%&\leq 2\cdot \opt + (1+ {2\over \beta}) \cdot \cost(S) &&\rhd \text{by Cauchy-Schwarz inequality} 
\end{align*}
\end{proof}
Since $S$ is a $(t,\eps)$-stable set of centers and all partitions in $\sQ$ are of size at most $t$ (i.e., $|S(Q)|\leq t$), 
for each $Q\in \sQ$, $\sum_{x\in P} \d(x, S_Q) - \d(x, S) \geq -\eps \cdot \cost(S)$. 
Hence, together with Claim~\ref{clm:bound-R-term} and Eq.~\eqref{eq:final-bound}, 
\begin{align}
-\eps |\sQ| \cost(S)  
&\leq \sum_{Q\in \sQ} \sum_{x\in P} \d(x, S_Q) - \d(x, S) \nonumber\\
&\leq \gamma\cdot \opt - (\gamma\cdot\Delta + 1) \cdot \cost(S) + \gamma\cdot \Delta \cdot \sum_{x\in P} \d(x, s_{o_x}) &&\rhd\text{by Eq.~\eqref{eq:final-bound}} \nonumber \\
&\leq \gamma\cdot \opt - (\gamma\cdot\Delta + 1) \cdot \cost(S) + \gamma\cdot \Delta \cdot (2+\beta)^2\cdot \opt
%&\leq \sum_{Q\in \sQ} \sum_{x\in P} \d(x, S_Q) - \d(x, S) \nonumber\\
%&\leq \gamma (4\Delta +1) \opt - (1- {4\gamma \Delta \over \beta}) \cost(S) &&\rhd\text{by Eq.~\eqref{eq:final-bound} and Claim~\ref{clm:bound-R-term}}\label{eq:last-step}
\end{align}
Since $|\sQ| \leq k\cdot \gamma$, by setting $\eps =1/(2k\cdot \gamma)$, $-\eps |\sQ| \cost(S) \geq -\cost(S)/2$.
Hence, together with the assumption $\beta^2 = {\cost(S) / \opt}$,
\begin{align}
\beta^2  = {\cost(S) \over \opt} \leq {\gamma (1 + \Delta\cdot (2+\beta)^2) \over {1\over 2} + {\gamma\cdot \Delta}}
\end{align}
which implies that 
\begin{align}
&({1\over 2} + \gamma\cdot \Delta) \cdot \beta^2 \leq \gamma + \gamma\cdot \Delta \cdot (\beta^2 + 4\beta + 4) \nonumber \\
\Rightarrow\; &{\beta^2 \over 2} - 4\gamma\Delta\beta - \gamma (1+4\Delta) \leq 0 \label{eq:quadratic-form}
\end{align}


By solving the quadratic formula~\eqref{eq:quadratic-form}, $\beta\leq 4\gamma\Delta + \sqrt{(4\gamma\Delta)^2 + 2\gamma(4\Delta+1)} < 8\gamma\Delta + 2\gamma$. Hence, at the time local search terminates, $\cost(S) < 4\gamma^2\cdot (4\Delta+1)^2 \cdot \opt$.
\end{proof}

\begin{corollary}[restatement of Theorem \ref{thm:main} for $k$-means]
The local search algorithm with swaps of size at most $4$ returns a $(O(1),7)$-bicriteria approximate solution of $\alpha$-fair $k$-means of a point set $P$ of size $n$ in time $\tldO(k^{5} n^4)$.
\end{corollary}
\begin{proof}
By Lemma~\ref{lem:clustering-with-partition-fair}, the result of our local search algorithm returns a $(7\alpha)$-fair $k$-clustering. By Lemma~\ref{lem:means-constant} and the existence of a pair of $3$-bounded mapping and $(4,6)$-bounded covering (see Lemma~\ref{lem:stable-mapping} and~\ref{lem:stable-partitioning}), the $k$-means cost of the returned clustering is $O(\opt)$ where $\opt$ is the cost of an optimal $\alpha$-fair $k$-means of $P$. 

Finally, as we set $\eps = O(1/k)$ and by Theorem~\ref{thm:iterations} the runtime of the algorithm is $\tldO(k^5 n^4)$.
\end{proof}


\subsection{Empirical Evaluation of Local Search for $k$-Means}\label{sec:experiment-k-means}
Figures \ref{fig:fair-means} and \ref{fig:cost-means} show empirical comparisons of algorithms \textsc{FairKCenter}, local search with 1-swap and greedy (see Section~\ref{sec:experiments}) both in terms of fairness and the $k$-means cost of their solutions.

\begin{figure*}[!h]
\minipage{0.33\textwidth}
		\includegraphics[width=\textwidth]{plots/means/1.pdf}
  %\label{fig:diabetes}
\endminipage\hfill
\minipage{0.33\textwidth}
		\includegraphics[width=\textwidth]{plots/means/2.pdf}
  %\label{fig:bank}
\endminipage\hfill
\minipage{0.33\textwidth}%
		\includegraphics[width=\textwidth]{plots/means/3.pdf}
  %\label{fig:census}
\endminipage
\caption{Comparison of the fairness guarantees of the described algorithms for fair $k$-means on data sets Diabetes, Bank and Census.}
\label{fig:fair-means}
\end{figure*}


The plots show that local-search based algorithms perform reasonably well with respect to the notion of $\alpha$-fairness: While its fairness guarantee is close to the fairness of \textsc{FairKCenter}, it always exhibits a better performance in terms of $k$-means cost. 
More precisely, on average the local search algorithm reports a solution whose cost is better than the algorithm of \cite{jung2019center} by a factor of 2.93, 2.32, and 1.73  
while the reported solution has a worse fairness by a factor of 1.14, 1.85, and 1.48 for Diabetes, Bank and Census respectively.



\begin{figure*}[!h]
\minipage{0.33\textwidth}
		\includegraphics[width=\textwidth]{plots/means/4.pdf}
  %\label{fig:diabetes}
\endminipage\hfill
\minipage{0.33\textwidth}
		\includegraphics[width=\textwidth]{plots/means/5.pdf}
  %\label{fig:bank}
\endminipage\hfill
\minipage{0.33\textwidth}%
		\includegraphics[width=\textwidth]{plots/means/6.pdf}
  %\label{fig:census}
\endminipage
\caption{Comparison of the $k$-means cost of the described algorithms for fair $k$-means on data sets Diabetes, Bank and Census.}
\label{fig:cost-means}
\end{figure*}

